What leads to generalization of object proposals?

Object proposal generation is often the first step in many detection models. It is lucrative to train a good proposal model, that generalizes to unseen classes. This could help scaling detection models to larger number of classes with fewer annotations. Motivated by this, we study how a detection model trained on a small set of source classes can provide proposals that generalize to unseen classes. We systematically study the properties of the dataset - visual diversity and label space granularity - required for good generalization. We show the trade-off between using fine-grained labels and coarse labels. We introduce the idea of prototypical classes: a set of sufficient and necessary classes required to train a detection model to obtain generalized proposals in a more data-efficient way. On the Open Images V4 dataset, we show that only 25% of the classes can be selected to form such a prototypical set. The resulting proposals from a model trained with these classes is only 4.3% worse than using all the classes, in terms of average recall (AR). We also demonstrate that Faster R-CNN model leads to better generalization of proposals compared to a single-stage network like RetinaNet.

==> experiments_model.tex <==
\subsection{Modeling Choices}
We first identify the best detection model and settings to extract proposals that generalize to new unseen classes. We then analyze generalization ability under different settings from this model. We reiterate that in order to test generalization, evaluation is done on target classes that have no intersection with the source classes used during training.

\noindent {\textbf{Choice of detection model:}} We compare the ability of a two-stage network (\frcnn) and a single-stage network (Retinanet) trained on a set of seen classes to generalize to new unseen classes in Fig.~\ref{fig:mod1}. We also show the performance of the respective models on the seen classes as well. The difference in performance between seen and unseen classes can be viewed as the generalization gap for the respective models. Since, in a two-stage model like \frcnn, the output from the RPN is class-agnostic and can be used as proposals too, we report the performance of the RPN as well.

\noindent {\textbf{Comparison with Region Proposal Network:}}
The results so far where obtained using class specific bounding box regression (which is the standard setting in \frcnn) for the detection head. Since we want the bounding boxes to generalize to unseen classes, class agnostic regression could be a valid choice too. We study this in Table~\ref{tab:class_agnostic} for \oiv and \coco.

First we see that class agnostic regression is comparable, or provides a slightly higher \AR{K} for small values of $K < 100$. However, when we consider more proposals (\AR{1000}), class specific regression provides a significant gain ($4.5\%$ for \oiv and $7.5\%$ for \coco). It results in multiple regressed versions (one corresponding to each class) of the same proposal generated from the RPN head. This helps in improving recall at higher values of $K$ but could be less helpful when $K$ is small. This is an important design consideration depending on the value of $K$ needed an application. 

In previous experiments, we fixed the the NMS threshold to $0.5$ to generate proposals. However, NMS threshold could have an impact on the quality of the proposals. We study the effect of NMS threshold in Figure~\ref{fig:nms_fig} for \oiv and \coco. We again train on \oivsource, \cocosource and test on \oivtarget, \cocotarget respectively. We report \AR{K} for different values of $K$.


We observe that for smaller number of proposals ($K < 100$), lower thresholds tend to provide the best results. Intuitively, a low threshold can improve spatial coverage of objects since proposals are well spread out. When considering a larger number of proposals ($K > 100$), there are sufficient boxes to ensure spatial coverage, and having some redundancy is helpful. This is witnessed by the drop in $\AR{100,1000}$ at low NMS thresholds.


\begin{figure}[!tbp]
  \centering
  \begin{minipage}[t]{0.46\textwidth}
    \includegraphics[width=\textwidth]{figures/cls_specific_vs_agnostic.pdf}
    \caption{Effect of class agnostic regression vs. class specific regression when using detections as proposals}
    \label{fig:cls_ag}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.46\textwidth}
    \includegraphics[width=\textwidth]{figures/oiv4_nms.pdf}
    \caption{Effect of NMS threshold on performance of proposals}
    \label{fig:nms_fig}
  \end{minipage}
  \vspace*{-0.25in}
\end{figure}


% \noindent {\textbf{Comparison with Region Proposal Network:}} In a two-stage model like \frcnn, the output from the RPN is class-agnostic and can be used as proposals too. Further, one could expect the RPN to be less-sensitive to missing bounding boxes in 

In Fig.~\ref{fig:rpn_vs_det}, we compare the performance of the RPN (from \frcnn) with the detection head of \frcnn and a single stage network like Retinanet. For combining the detections, we use NMS and class score thresholds of $0.5$ and $0.0$ respectively. To get an upper bound, we combine data from source and target classes to train a detector (denoted by Source: \oivall and Source: \cocoall in Fig.~\ref{fig:rpn_vs_det}). The performance of the RPN and detector head of a \frcnn trained with this full dataset is shown in the figures.

\begin{figure}[t]
  \begin{minipage}[t]{0.60\textwidth}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/oiv4_rpn_vs.pdf}
        \caption{OIV4}
        \label{fig:1}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/oiv4_rpn_vs.pdf}
        \caption{COCO}
        \label{fig:2}
    \end{subfigure}
    \caption{Comparing proposals from RPN head and detection head for the OIV4and COCO dataset}
    \label{fig:rpn_vs_det}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/coco_ar_breakdown_v2.pdf}
    \caption{\AR{1000} on \cocotarget is shown for different IoU thresholds for both RPN and Detection heads}
    \label{fig:nms_fig}
  \end{minipage}
\end{figure}

% We observe that detection heads from \frcnn and Retinanet, both significantly outperform the RPN head on both datasets (\oivsource and \cocosource columns) for unseen classes. This shows that the boxes from the detection head generalize to unseen classes in the target dataset better. We also note that Retinanet and \frcnn yield comparable performances. Hence, we expect the observations made with \frcnn to transfer to single stage networks like Retinanet and we fix \frcnn as the base model for all analysis from now on, unless specified otherwise.

% %Specifically, \AR{100} improves from $55.0\%$ to $69.4\%$ for \oiv and $31.5\%$ to $44.0\%$ for \coco for unseen classes.

% The superior performance of the detection head can be attributed to better bounding box regression from the detection head which has additional layers, following the RPN in the model. To investigate this effect, we measure \AR{1000} at different IoU thresholds for both sets of proposals for the model trained on \cocosource and evaluated on \cocotarget in Fig.~\ref{fig:nms_fig}. We see that the difference increases drastically at higher values of IoU threshold, and is negligible at a threshold of $0.5$. This implies that the boxes from the detection head are more fine-tuned to exactly localize the objects.


\noindent {\textbf{Weakly supervised detection:}}
A strong practical utility for generalized proposals is that, no bounding box annotations should be needed to train a detection model for new object classes. Hence, we report the performance of a weakly supervised detection model (that does not use bounding box annotations) trained with the proposals in Tab.~\ref{tab:det_map}. The model is trained on \oivtarget-train and evaluated on \oivtarget-test. We show results for proposals obtained from training with \oivsource as well as \oivall. We see that the performance of the weakly supervised detection model is directly correlated with the generalization ability of the proposals being used, showing the need for good generalized proposals.

% . The better proposals obtained from the detection head lead to higher AP

\begin{table}[t]
%\vspace{-0.1in}
\scriptsize
% \setlength\extrarowheight{1.0pt}
\centering
\begin{center}
\caption{Comparing performance of proposals generated by RPN head and detection head for weakly supervised detection. We also show the \AR{100} numbers which are seen to be correlated with detection AP. Det. refers to Detection}\label{tab:det_map}
\begin{tabular}{|P{1.3cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|}
\hline
\multicolumn{5}{|c|}{Target Dataset - \oivtarget}\\
\hline
 & \multicolumn{2}{c|}{Source: \oivsource} & \multicolumn{2}{c|}{Source: \oivall}\\
& Det. AP & \AR{100} & Det. AP & \AR{100} \\\hline
RPN head & 8.7 & 55.0 & 9.6 & 60.4\\
Det. head & \textbf{24.0} & \textbf{69.4} & \textbf{30.8} & \textbf{76.9} \\
\hline

\end{tabular}
\end{center}
\vspace{-0.2in}
%\vspace{-0.2in}
\end{table}

% \noindent {\textbf{Class specific regression and NMS threshold:}}
% The results so far where obtained using class specific bounding box regression (which is the standard setting in \frcnn) for the detection head. Since we want the bounding boxes to generalize to unseen classes, class agnostic regression could be a valid choice too. We study this in Table~\ref{tab:class_agnostic} for \oiv and \coco.

% First we see that class agnostic regression is comparable, or provides a slightly higher \AR{K} for small values of $K < 100$. However, when we consider more proposals (\AR{1000}), class specific regression provides a significant gain ($4.5\%$ for \oiv and $7.5\%$ for \coco). It results in multiple regressed versions (one corresponding to each class) of the same proposal generated from the RPN head. This helps in improving recall at higher values of $K$ but could be less helpful when $K$ is small. This is an important design consideration depending on the value of $K$ needed an application. 

% In previous experiments, we fixed the the NMS threshold to $0.5$ to generate proposals. However, NMS threshold could have an impact on the quality of the proposals. We study the effect of NMS threshold in Figure~\ref{fig:nms_fig} for \oiv and \coco. We again train on \oivsource, \cocosource and test on \oivtarget, \cocotarget respectively. We report \AR{K} for different values of $K$.


% We observe that for smaller number of proposals ($K < 100$), lower thresholds tend to provide the best results. Intuitively, a low threshold can improve spatial coverage of objects since proposals are well spread out. When considering a larger number of proposals ($K > 100$), there are sufficient boxes to ensure spatial coverage, and having some redundancy is helpful. This is witnessed by the drop in $\AR{100,1000}$ at low NMS thresholds.


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[t]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/cls_specific_vs_agnostic.pdf}
%     \caption{Effect of class agnostic regression vs. class specific regression when using detections as proposals}
%     \label{fig:cls_ag}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/oiv4_nms.pdf}
%     \caption{Effect of NMS threshold on performance of proposals}
%     \label{fig:nms_fig}
%   \end{minipage}
% \end{figure}


==> intro.tex <==
\section{Introduction}
\label{sec:intro}
Object detection systems have shown considerable improvements for the fully supervised setting \cite{ren2015faster,lin2017focal,liu2016ssd} on challenging benchmarks like COCO~\cite{coco} with large number of bounding box annotations for each class. Since annotating bounding boxes is a tedious time consuming process, weakly supervised methods~\cite{Gao_2019_ICCV,arun2019dissimilarity,tang2018pcl} that only use image-level labels are gaining increasing attention as well. 

Both approaches typically consider detection as a combination of two tasks: (a) spatial localization of the object in an image using a bounding box (proposals) and (b) classification of the bounding box into the correct category. One way to scale object detection to a large number of classes would be to develop a good class-agnostic localization model that \emph{generalizes} to all classes. We could then train more data efficient detection models, requiring fewer or no bounding box annotations to only solve the classification task. Recent works \cite{uijlings2018revisiting,singh2018r} have also shown the benefit of good proposal models for training object detectors with limited bounding box annotations.

In our work, we study this notion of a generalized proposal model. In other words, how well can an object localization model trained on a small set of classes also localize other unseen classes? Intuitively, to localize a fine-grained vehicle like taxi, it might be sufficient to train a localization model with examples from other vehicles like cars or vans (as shown in Fig.~\ref{fig:pull_fig}). For localization (unlike classification), we may not need any training data for this class. While there have been few works that leverage this intuition for weakly supervised learning~\cite{uijlings2018revisiting}, the extent to which object localization depends on the categories used to train the localization model has not been well quantified and studied in detail. For example, does the above example extend beyond fine-grained categories? Can a model trained on cars localize other vehicles?
% For example, does this extend beyond fine-grained categories? Can a model trained on cars localize other vehicles?  

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures/rui_pull}
\caption{Proposal models learned on source vehicle classes can localize unseen target objects which share similar localization structure like ``bus" and ``taxi". However, ``barge" and ``gondola", which are also vehicles will not be localized by this model, due to lack of visual diversity in the source dataset for vehicles}
\label{fig:pull_fig}
\vspace{-0.2in}
\end{figure}


We show that with \emph{careful design considerations}, it is possible to train a good "generalized proposal model". The main contribution of our work is two-fold: a) We formally and systematically study the desired properties of a dataset required to build such a model, and b) We highlight critical modeling and hyper-parameter choices that enable us to leverage existing  frameworks like \frcnn~\cite{ren2015faster}.

We answer several key questions regarding the \emph{dataset}:

\noindent {\bf{Label Space Granularity: }}We show that annotating bounding boxes with coarse (e.g. vehicle rather than sports car in Fig.~\ref{fig:pull_fig}) labels is sufficient to get good proposals. Getting these coarse-grained annotations are significantly less tedious and more accurate than the fine-grained ones.

%Our observations are in line with previous works~\cite{uijlings2018revisiting,singh2018r}, but differ in precisely quantifying the requied level of granularity.
\noindent {\bf{Semantic and Visual Diversity: }}We observe that it is crucial to have semantic and visual diversity at both coarse and fine levels of granularity for good generalization. For instance, when training a proposal model with a coarse label "vehicle", we need examples of different types of vehicles like "car" and "boats", even if the examples are only annotated as ``vehicle" as shown in Fig.~\ref{fig:pull_fig}. But are all classes within a coarse category equally important? This question is important to answer since sourcing data from a large number of fine-grained categories is very challenging.
To this end, we introduce the concept of {\it{prototypical classes}} as a subset of leaf classes in a semantic hierarchy that are sufficient and necessary to construct a dataset to train a good generalized proposal model. We show that it is indeed possible to construct a small prototypical set. This has positive implications for large taxonomies, since it is sufficient to annotate examples only for the prototypical classes. We also study different empirical ways of identifying these classes.

%\noindent {\bf{Semantic and Visual Diversity: }}We observe that even at a coarse granularity, it is crucial to have visual diversity among the objects covered under each coarse label. For instance, when training a proposal model with the coarse label "vehicle", we need examples of different types of vehicles like "car" and "aeroplane", even if the examples are only annotated as "vehicle".\dhruv{This contradicts the prototypical classe paragraph below.. we need to change it totally.}
%We further analyze how much importance should be paid to collect data from the diverse set of objects in each coarse category. To this end, we introduce the concept of {\it{prototypical classes}} as a subset of leaf classes in a semantic hierarchy that are sufficient to construct a dataset to train a good generalized proposal model. We empirically study different ways of identifying the prototypical leaf classes and show that a small prototypical set is sufficient. This has positive implications for large taxonomies, since it is sufficient to annotate examples only for the prototypical classes.\dhruv{Paragraph needs rewording.}

%This has positive implications for constructing generalized proposal model for very big taxonomies in future and is one of the main contributions of our work.

%We give an empirical existential proof that a small set of prototypical leaf classes is sufficient to build a good model. 

We also propose key \emph{modeling} choices that are critical for leveraging state-of-the-art detectors like \frcnn to obtain generalized proposals. We observe that the detections from a \frcnn model serve as better generalized proposals than the outputs from its Region Proposal Network (RPN). We also show the effect of NMS threshold and class agnostic regression in generating good proposals.  

On \oiv \cite{kuznetsova2018open} dataset, we show a significant improvement of $9\%-13\%$ in the average recall (\AR{k}) of proposals, when using detections rather than RPN outputs for generalized proposals. We observe that coarse-grained labels are sufficient to train a good proposal model that generalizes to all the \oiv classes. Finally, compared to training with all the seen objects, we show that training with less than $25\%$ of the object classes chosen appropriately leads to only a drop of $4.3\%$ in \AR{100}, while training with $50\%$ of such classes leads to a negligible drop of $0.9\%$.

==> old_experiments_model.tex <==

 %We would expect the detection performance to be correlated with \AR{100}.
%We found this to yield better detection performance than using the entire set of proposals. 


\subsection{Modeling Choices}
We first identify the best way to extract proposals that generalize to new unseen classes, from a detection model. We analyze bounding boxes obtained under different settings from a detection model.  We reiterate that evaluation is done on target classes that have no intersection with the source classes used during training.

\noindent {\textbf{Proposals from detection model:}} As we showed in Sec.~\ref{subsec:model}, bounding boxes from a detection model can be combined in a class-agnostic fashion to obtain proposals. However, in a two-stage model like \frcnn, the output from the RPN is class-agnostic and can be used as proposals too. In Fig.~\ref{fig:rpn_vs_det}, we compare the performance of the RPN (from \frcnn) with the detection head of \frcnn and a single stage network like Retinanet. For combining the detections, we use NMS and class score thresholds of $0.5$ and $0.0$ respectively. To get an upper bound, we combine data from source and target classes to train a detector (denoted by Source: \oivall and Source: \cocoall in Fig.~\ref{fig:rpn_vs_det}). The performance of the RPN and detector head of a \frcnn trained with this full dataset is shown in the figures.

\begin{figure}[t]
  \begin{minipage}[t]{0.60\textwidth}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/oiv4_rpn_vs.pdf}
        \caption{OIV4}
        \label{fig:1}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/oiv4_rpn_vs.pdf}
        \caption{COCO}
        \label{fig:2}
    \end{subfigure}
    \caption{Comparing proposals from RPN head and detection head for the OIV4and COCO dataset}
    \label{fig:rpn_vs_det}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/coco_ar_breakdown.pdf}
    \caption{\AR{1000} on \cocotarget is shown for different IoU thresholds for both RPN and Detection heads}
    \label{fig:nms_fig}
  \end{minipage}
\end{figure}

% \begin{table} %[t]
% %\vspace{-0.1in}
% \scriptsize
% % \setlength\extrarowheight{1.0pt}
% \setlength{\tabcolsep}{4pt}
% \centering
% \begin{center}
% \caption{Comparing proposals from RPN head and detection head for the OIV4 and COCO datasets. \oivall refers to training by combining data both from source and target classes, and proposal models trained with this data serves as a good upper bound for generalization}
% \begin{tabular}{|P{1.35cm}|P{0.89cm}|P{0.89cm}|P{0.89cm}|P{0.89cm}|}
% \hline
% \multicolumn{5}{|c|}{Target Dataset - \oivtarget}\\
% \hline
%  & \multicolumn{2}{c|}{Source: \oivsource} & \multicolumn{2}{c|}{Source: \oivall}\\
% Head Type & \AR{100} & \AR{1000} & \AR{100} & \AR{1000} \\\hline
% RPN & 55.0 & 61.9 & 60.4 & 65.0\\
% Detection & 69.4 & 80.5 & 76.9 & 84.4\\
% \hline \hline
% \multicolumn{5}{|c|}{Target Dataset - \cocotarget}\\
% \hline
%  & \multicolumn{2}{c|}{Source: \cocosource} & \multicolumn{2}{c|}{Source: \cocoall}\\
% Head Type & \AR{100} & \AR{1000} & \AR{100} & \AR{1000} \\\hline
% RPN & 31.5 & 47.9 & 46.9 & 58.7 \\
% Detection & 44.0 & 58.0 & 59.9 & 68.9 \\
% \hline
% \end{tabular}
% \end{center}
% %\vspace{-0.1in}
% \label{tab:det_as_proposals}
% %\vspace{-0.2in}
% \end{table}

We observe that detection heads from \frcnn and Retinanet, both significantly outperform the RPN head on both datasets (\oivsource and \cocosource columns) for unseen classes. This shows that the boxes from the detection head generalize to unseen classes in the target dataset better. We also note that Retinanet and \frcnn yield comparable performances. Hence, we expect the observations made with \frcnn to transfer to single stage networks like Retinanet and we fix \frcnn as the base model for all analysis from now on, unless specified otherwise.

%Specifically, \AR{100} improves from $55.0\%$ to $69.4\%$ for \oiv and $31.5\%$ to $44.0\%$ for \coco for unseen classes.

The superior performance of the detection head can be attributed to better bounding box regression from the detection head which has additional layers, following the RPN in the model. To investigate this effect, we measure \AR{1000} at different IoU thresholds for both sets of proposals for the model trained on \cocosource and evaluated on \cocotarget in Fig.~\ref{fig:nms_fig}. We see that the difference increases drastically at higher values of IoU threshold, and is negligible at a threshold of $0.5$. This implies that the boxes from the detection head are more fine-tuned to exactly localize the objects.

%This can be attributed to the fact that the detection head has additional layers, leading to better bounding box regression.

% \begin{table}
% %\vspace{-0.1in}
% \scriptsize
% % \setlength\extrarowheight{1.0pt}
% \setlength{\tabcolsep}{4pt}
% \centering
% \begin{center}
% \caption{\AR{1000} on \cocotarget is shown for different IoU thresholds for both RPN and Detection heads} \label{tab:box_vs_scores}
% \begin{tabular}{|P{1.1cm}|P{1.1cm}|P{0.6cm}|P{.6cm}|P{.6cm}|P{.6cm}|P{.7cm}|}
% \hline
% & \AR{1000} & AR$_{0.5}$ & AR$_{0.6}$ & AR$_{0.7}$ & AR$_{0.8}$ & AR$_{0.9}$ \\
% \hline
% RPN head & 47.9 & 81.9 & 75.9 & 64.0 & 33.0 & 4.7 \\ \hline
% Det. head & 58.0 & 82.4 & 77.6 & 69.4 & 54.5 & 27.4 \\
% \hline
% \end{tabular}
% \end{center}
% %\vspace{-0.1in}
% %\vspace{-0.2in}
% \end{table}


\noindent {\textbf{Weakly supervised detection:}}
A strong practical utility for developing generalized proposals that localize all objects is that, no bounding box annotations should be needed to train a detection model for new object classes. Hence, we also report the performance of a weakly supervised detection model (that does not need any bounding box annotations) trained with the proposals in Table~\ref{tab:det_map}. The weakly supervised model is trained on \oivtarget-train and evaluated on \oivtarget-test. We show results for proposals obtained from training with \oivsource as well as \oivall. We see that the performance of the weakly supervised detection model is directly correlated with the generalization ability of the proposals being used. The better proposals obtained from the detection head lead to higher AP, showing the need for good generalized proposals.

\begin{table}[t]
%\vspace{-0.1in}
\scriptsize
% \setlength\extrarowheight{1.0pt}
\centering
\begin{center}
\caption{Comparing performance of proposals generated by RPN head and detection head for weakly supervised detection. We also show the \AR{100} numbers which are seen to be correlated with detection AP. Det. refers to Detection}\label{tab:det_map}
\begin{tabular}{|P{1.3cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|}
\hline
\multicolumn{5}{|c|}{Target Dataset - \oivtarget}\\
\hline
 & \multicolumn{2}{c|}{Source: \oivsource} & \multicolumn{2}{c|}{Source: \oivall}\\
& Det. AP & \AR{100} & Det. AP & \AR{100} \\\hline
RPN head & 8.7 & 55.0 & 9.6 & 60.4\\
Det. head & \textbf{24.0} & \textbf{69.4} & \textbf{30.8} & \textbf{76.9} \\
\hline

\end{tabular}
\end{center}
\vspace{-0.2in}
%\vspace{-0.2in}
\end{table}

\noindent {\textbf{Class specific regression and NMS threshold:}}
The results so far where obtained using class specific bounding box regression (which is the standard setting in \frcnn) for the detection head. Since we want the bounding boxes to generalize to unseen classes, class agnostic regression could be a valid choice too. We study this in Table~\ref{tab:class_agnostic} for \oiv and \coco.

% \begin{table}[t]
% %\vspace{-0.1in}
% \scriptsize
% % \setlength\extrarowheight{1.0pt}
% \setlength{\tabcolsep}{4pt}
% \centering
% \begin{center}
% \caption{Effect of class agnostic regression vs. class specific regression when using detections as proposals} \label{tab:class_agnostic}
% \begin{tabular}{|P{1.8cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}|P{1.0cm}|}
% \hline
% \multicolumn{6}{|c|}{Source Dataset - \oivsource, Target Dataset - \oivtarget}\\
% \hline 
% bbox reg & \AR{10} & \AR{20} & \AR{50} & \AR{100} & \AR{1000} \\
% \hline
% cls-specific & 49.1 & 54.0 & 59.8 & 64.2 & \textbf{76.1} \\
% \hline
% cls-agnostic & \textbf{49.9} & \textbf{55.2} & \textbf{60.8} & \textbf{64.5} & 68.6 \\
% \hline
% \multicolumn{6}{|c|}{Source Dataset - \cocosource, Target Dataset - \cocotarget}\\
% \hline
% cls-specific & 24.4 & 29.2 & 37.1 & 43.8 & \textbf{59.4} \\
% \hline
% cls-agnostic & \textbf{25.9} & \textbf{30.8} & \textbf{38.9} & \textbf{45.2} & 54.9 \\
% \hline
% \end{tabular}
% \end{center}
% %\vspace{-0.1in}

% %\vspace{-0.2in}
% \end{table}

First we see that class agnostic regression is comparable, or provides a slightly higher \AR{K} for small values of $K < 100$. However, when we consider more proposals (\AR{1000}), class specific regression provides a significant gain ($4.5\%$ for \oiv and $7.5\%$ for \coco). It results in multiple regressed versions (one corresponding to each class) of the same proposal generated from the RPN head. This helps in improving recall at higher values of $K$ but could be less helpful when $K$ is small. This is an important design consideration depending on the value of $K$ needed an application. 

In previous experiments, we fixed the the NMS threshold to $0.5$ to generate proposals. However, NMS threshold could have an impact on the quality of the proposals. We study the effect of NMS threshold in Figure~\ref{fig:nms_fig} for \oiv and \coco. We again train on \oivsource, \cocosource and test on \oivtarget, \cocotarget respectively. We report \AR{K} for different values of $K$.

%  Having a very high threshold could lead to redundant boxes, while a low threshold could reduce coverage of adjacent objects in an image. 

% \begin{figure}
% \centering
% \includegraphics[scale=0.28]{figures/effect_of_nms.pdf}
% \caption{Effect of NMS threshold on performance of proposals \label{fig:nms_fig}}
% \end{figure}

We observe that for smaller number of proposals ($K < 100$), lower thresholds tend to provide the best results. Intuitively, a low threshold can improve spatial coverage of objects since proposals are well spread out. When considering a larger number of proposals ($K > 100$), there are sufficient boxes to ensure spatial coverage, and having some redundancy is helpful. This is witnessed by the drop in $\AR{100,1000}$ at low NMS thresholds.

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[t]{0.30\textwidth}
%     \includegraphics[width=\textwidth]{figures/oiv4_rpn_vs.pdf}
%     \caption{Effect of class agnostic regression vs. class specific regression when using detections as proposals}
%     \label{fig:cls_ag}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.30\textwidth}
%     \includegraphics[width=\textwidth]{figures/oiv4_rpn_vs.pdf}
%     \caption{Effect of NMS threshold on performance of proposals}
%     \label{fig:nms_fig}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{figures/coco_ar_breakdown.pdf}
%     \caption{Effect of NMS threshold on performance of proposals}
%     \label{fig:nms_fig}
%   \end{minipage}
% \end{figure}


\begin{figure}[!tbp]
  \centering
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/cls_specific_vs_agnostic.pdf}
    \caption{Effect of class agnostic regression vs. class specific regression when using detections as proposals}
    \label{fig:cls_ag}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/oiv4_nms.pdf}
    \caption{Effect of NMS threshold on performance of proposals}
    \label{fig:nms_fig}
  \end{minipage}
\end{figure}

